Heterogeneous Federated Learning with Splited Language Model

Federated Split Learning (FSL) is a promising distributed learning paradigm in practice, which gathers the strengths of both Federated Learning (FL) and Split Learning (SL) paradigms, to ensure model privacy while diminishing the resource overhead of each client, especially on large transformer models in a resource-constrained environment, e.g., Internet of Things (IoT). However, almost all works merely investigate the performance with simple neural network models in FSL. Despite the minor efforts focusing on incorporating Vision Transformers (ViT) as model architectures, they train ViT from scratch, thereby leading to enormous training overhead in each device with limited resources. Therefore, in this paper, we harness Pre-trained Image Transformers (PITs) as the initial model, coined FedV, to accelerate the training process and improve model robustness. Furthermore, we propose FedVZ to hinder the gradient inversion attack, especially having the capability compatible with black-box scenarios, where the gradient information is unavailable. Concretely, FedVZ approximates the server gradient by utilizing a zeroth-order (ZO) optimization, which replaces the backward propagation with just one forward process. Empirically, we are the first to provide a systematic evaluation of FSL methods with PITs in real-world datasets, different partial device participations, and heterogeneous data splits. Our experiments verify the effectiveness of our algorithms.

==> 2_pre.tex <==
\section{Preliminary}


==> 7_analysis.tex <==
\section{Theoretical Analysis}\label{th}
\begin{assumption} \label{Lipschitzian_gradient}
(Lipschitz Smoothness). The function $f_i$ is differentiable and $\nabla f_i$ is $L$-Lipschitz continuous, $\forall i \in \{1,2,\ldots,M\}$, i.e.,
$\|\nabla f_i( x) - \nabla f_i( y)\| \leq L \|x-y\|,$
for all $x, y \in \mathbb{R}^d$.
% The first-order Lipschitz assumption is commonly used in the ML community. Here, for simplicity, we suppose all functions enjoy the same Lipschitz constant $L$.
\end{assumption}


\begin{assumption} \label{local_Bounded_variance}
(Local Bounded Variance). The gradient of the function $f_i$ have $\sigma_l$-bounded variance:
\begin{equation}
\small
			\mathbb{E}_{\xi_c}\left\|\nabla f_i (w;\xi_c ) -\nabla f_i (w)\right  \|^2 \leq \sigma_l^2, \forall i \in \{1,2,\ldots,M\},\nonumber
\end{equation}   
for each client $i$ with all $w \in \mathbb{R}^d$. 
\end{assumption}

\begin{assumption} \label{global_Bounded_variance}
(Global Bounded Variance). The gradient of the function $f_i$ have $\sigma_l$-bounded variance:
\begin{equation}
\small
	\|\nabla f_i(w) - \nabla F(w)\|^2 \leq \sigma_{g}^2,\nonumber
\end{equation}
and the global variance is also bounded, i.e.,  for all $w \in \mathbb{R}^d$. Note that the value of $\sigma_g^2$ indicates the degree of non-IID, which means the situation of data heterogeneity.
\end{assumption}
